Self-Supervised Coordinate Projection Network for Sparse-View Computed Tomography

In the present work, we propose a Self-supervised COordinate Projection nEtwork (SCOPE) to reconstruct the artifacts-free CT image from a single SV sinogram by solving the inverse tomography imaging problem. Compared with recent related works that solve similar problems using implicit neural representation network (INR), our essential contribution is an effective and simple re-projection strategy that pushes the tomography image reconstruction quality over supervised deep learning CT reconstruction works. The proposed strategy is inspired by the simple relationship between linear algebra and inverse problems. To solve the under-determined linear equation system, we first introduce INR to constrain the solution space via image continuity prior and achieve a rough solution. And secondly, we propose to generate a dense view sinogram that improves the rank of the linear equation system and produces a more stable CT image solution space. Our experiment results demonstrate that the re-projection strategy significantly improves the image reconstruction quality (+3 dB for PSNR at least). Besides, we integrate the recent hash encoding into our SCOPE model, which greatly accelerates the model training. Finally, we evaluate SCOPE in parallel and fan X-ray beam SVCT reconstruction tasks. Experimental results indicate that the proposed SCOPE model outperforms two latest INR-based methods and two well-popular supervised DL methods quantitatively and qualitatively.

==> table/ablation_re-projection_table.tex <==
\begin{table*}[ht]
\centering
\caption{Qualitative results (PSNR/SSIM/LPIPS) for the SCOPE++ model with four reconstruction settings on the COVID-19 dataset. The best performance are highlighted in \textbf{bold}.}
\label{table:ablation-reprojection}
\resizebox{0.80\linewidth}{!}{
\begin{tabular}{lccccc} 
\toprule
\textbf{X-rays}               & \textbf{Views} & \textbf{No Re.}     & \textbf{$K_d=360$}  & \textbf{720 Re. Views}  & \textbf{1440 Re. Views}  \\ 
\midrule\midrule
\multirow{3}{*}{\textbf{Parallel}} & $60$                   & $31.91/0.9378/0.0469$ & $35.30/0.9460/0.0208$ & ${\mathbf{35.36}}/0.9512/\mathbf{0.0196}$ & $35.32/\mathbf{0.9513}/0.0196$  \\ 

                                   & $90$                   & $34.70/0.9661/0.0207$ & $40.32/0.9771/0.0044$ & ${\mathbf{40.57}}/{\mathbf{0.9807}}/{\mathbf{0.0040}}$ & $40.54/0.9806/{\mathbf{0.0040}}$  \\ 

                                   & $120$                  & $35.35/0.9706/0.0173$ & $42.67/0.9841/0.0025$ & ${\mathbf{43.09}}/{\mathbf{0.9872}}/{\mathbf{0.0023}}$ & $43.05/0.9871/0.0024$  \\ 
\midrule
\multirow{3}{*}{\textbf{Fan}}      & $60$                   & $35.21/0.9616/0.0128$ & $35.84/0.9364/0.0230$ & ${\mathbf{37.93}}/{\mathbf{0.9727}}/{\mathbf{0.0067}}$ & $37.86/0.9718/0.0068$  \\ 

                                   & $90$                   & $36.90/0.9738/0.0074$ & $37.89/0.9488/0.0190$ & ${\mathbf{41.76}}/{\mathbf{0.9854}}/{\mathbf{0.0023}}$ & $41.53/0.9845/0.0024$  \\ 

                                   & $120$                  & $37.46/0.9769/0.0069$ & $38.53/0.9516/0.0188$ & ${\mathbf{43.62}}/{\mathbf{0.9888}}/{\mathbf{0.0015}}$ & $43.27/0.9878/0.0017$  \\
\bottomrule
\end{tabular}}
\end{table*}

==> table/hash_table.tex <==
\begin{table}[t]
\renewcommand\arraystretch{1.05}
\centering
\caption{Hyper-parameters of the hash encoding \cite{muller2022instant} used in SCOPE.}
\label{table-hash}
\resizebox{0.40\textwidth}{!}{
\begin{tabular}{llr} 
\toprule
\textbf{Hyper-Parameter}        & \textbf{Symbol} & \textbf{Value}  \\ 
\midrule
{Number of levels}                     & $L$                    & $8$                 \\
{Hash table size}                     & $T$                    & $2^{24}$                 \\
{Number of feature dimensions per entry}                     & $F$                    & $8$                 \\
{Coarsest resolution}                     & $N_{\text{min}}$                    & $2$                 \\
{Geometric growth factor}                     & $b$                    & $2$                 \\
\bottomrule
\end{tabular}}
\end{table}

==> table/recon_table.tex <==
\begin{table}[t]
\centering
\caption{Quantitative results (PSNR/SSIM) of the SCOPE model with three encoding modules on the COVID-19 dataset for \textit{parallel} and \textit{fan} X-rays beam SVCT of 60, 90, and 120 views. The best performances are highlighted in bold.}
\label{table:ablation-recon}
\resizebox{\linewidth}{!}{
\begin{tabular}{clccc}
\toprule
\textbf{X-ray}                & \textbf{Recon. Method} & \textbf{60 Views} & \textbf{90 Views} & \textbf{120 Views}  \\ 
\midrule
\multirow{3}{*}{\textit{Parallel}} & ART \cite{gordon1974tutorial}            & $34.90/0.9503$      & $39.13/0.9786$      & $40.99/0.9865$        \\
                                   & FBPConvNet \cite{FBPConvNet}          & $\mathbf{36.37/0.9593}$      & $37.85/0.9664$      & $38.22/0.9681$        \\
                                   & FBP \cite{fbp}          & $35.36/0.9512$      & $\mathbf{40.57/0.9807}$      & $\mathbf{43.09/0.9872}$        \\ 
\midrule
\multirow{3}{*}{\textit{Fan}}      & ART \cite{gordon1974tutorial}            & $36.68/0.9678$      & $39.51/0.9811$      & $40.37/0.9843$        \\
                                   & FBPConvNet \cite{FBPConvNet}          & $30.39/0.9111$      & $30.60/0.9154$      & $30.64/0.9164$        \\
                                   & FBP \cite{fbp}          & $\mathbf{37.93/0.9727}$      & $\mathbf{41.76/0.9854}$      & $\mathbf{43.62/0.9888}$        \\
\bottomrule
\end{tabular}}
\end{table}

==> table/table_pipelineab.tex <==
\begin{table}[ht]
\centering
\caption{\textcolor{red}{Quantitative comparison of the generated DV sinogram via the two pipelines shown in Fig. \ref{fig:fig_DV_sino_generation} on the COVID-19 dataset \cite{shakouri2021covid19} for fan X-ray beam SVCT of 60, 90, and 120 views. The best performances are highlighted in bold.}}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{cccc} 
\toprule
\textbf{Pipeline} & \textbf{60 Views} & \textbf{90 Views} & \textbf{120 Views}  \\ 
\midrule
A           & $\mathbf{56.48/0.9989}$      & $\mathbf{59.73/0.9995}$      & $\mathbf{61.14/0.9996}$        \\
B          & $53.24/0.9983$      & $54.45/0.9989$      & $54.85/0.9990$        \\
\bottomrule
\end{tabular}}
\label{table:table_pipelineab}
\end{table}

==> table/table_projection_swapping.tex <==
\begin{table}[t]
\centering
\caption{\textcolor{red}{Quantitative results (PSNR/SSIM) of the ablation study for the projection swapping operator on the COVID-19 dataset for fan X-rays beam SVCT of 60, 90, and 120 views. The best performances are highlighted in bold.}}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{cccc} 
\toprule
\textbf{Modules} & \textbf{60 Views} & \textbf{90 Views} & \textbf{120 Views}  \\ 
\midrule
w/o Proj. Swap.           & $37.90/0.9726$      & $41.60/0.9853$      & $43.31/0.9886$        \\
w/ Proj. Swap.          & $\mathbf{37.93/0.9727}$      & $\mathbf{41.76/0.9854}$      & $\mathbf{43.62/0.9888}$        \\
\bottomrule
\end{tabular}}
\label{table:projection_swapping}
\end{table}
